AstroAgents: A Multi-Agent AI for Hypothesis Generation from Mass Spectrometry Data

With upcoming sample return missions across the solar system and the increasing availability of mass spectrometry data, there is an urgent need for methods that analyze such data within the context of existing astrobiology literature and generate plausible hypotheses regarding the emergence of life on Earth. Hypothesis generation from mass spectrometry data is challenging due to factors such as environmental contaminants, the complexity of spectral peaks, and difficulties in cross-matching these peaks with prior studies. To address these challenges, we introduce AstroAgents, a large language model-based, multi-agent AI system for hypothesis generation from mass spectrometry data. AstroAgents is structured around eight collaborative agents: a data analyst, a planner, three domain scientists, an accumulator, a literature reviewer, and a critic. The system processes mass spectrometry data alongside user-provided research papers. The data analyst interprets the data, and the planner delegates specific segments to the scientist agents for in-depth exploration. The accumulator then collects and deduplicates the generated hypotheses, and the literature reviewer identifies relevant literature using Semantic Scholar. The critic evaluates the hypotheses, offering rigorous suggestions for improvement. To assess AstroAgents, an astrobiology expert evaluated the novelty and plausibility of more than a hundred hypotheses generated from data obtained from eight meteorites and ten soil samples. Of these hypotheses, 36% were identified as plausible, and among those, 66% were novel. Project website: https://astroagents.github.io/

==> Discussion.tex <==
\section{Summary and Discussion}

Traditional approaches to analyzing large datasets often fail to uncover nuanced patterns and generate sophisticated hypotheses, typically identifying only basic correlations and trends while missing deeper insights. To address these limitations, we developed a multi-agent framework that employs specialized AI agents, each bringing distinct expertise to the analysis. By carefully crafting prompts, providing relevant research context, and assigning focused analytical objectives to each agent, our system generates novel hypotheses that might be overlooked using conventional methods, as demonstrated in our analysis of mass spectrometry data using \emph{AstroAgents}.

\emph{AstroAgents} introduces a novel paradigm that leverages the capabilities of large language models (LLMs) to analyze mass spectrometry data for origin-of-life research. Although this paper primarily focuses on a gas chromatography dataset, our methodology is versatile and can be applied to a wide range of datasets. The comparative performance of Claude 3.5 Sonnet and Gemini 2.0 Flash reveals important insights about the trade-offs between contextual capacity and collaborative ability in multi-agent systems. Claude 3.5 Sonnet's superior performance in consistency and clarity suggests that stronger agent collaboration capabilities may be more valuable than expanded context windows for generating reliable scientific hypotheses. However, Gemini 2.0 Flash's higher novelty scores indicate that larger context windows might facilitate more creative connections across broader knowledge bases.

Despite these promising results, several limitations remain. The system's reliance on human expert evaluation to determine the novelty of hypotheses introduces subjectivity; future research should explore more objective criteria for hypothesis assessment. Furthermore, the system currently depends on pre-selected research papers for context, making its performance heavily reliant on the quality and relevance of the provided literature. Enhancements could include developing dynamic literature-selection capabilities, allowing the system to autonomously identify and incorporate relevant research based on emerging data patterns. \emph{AstroAgents} demonstrates considerable potential for broader applications across diverse domains requiring the interpretation of complex, high-dimensional data.

\subsubsection*{Acknowledgments}
This research was supported by the Parker H. Petit Institute for Bioengineering and Biosciences (IBB) interdisciplinary seed grant, the Institute of Matter and Systems (IMS) Exponential Electronics seed grant, and the Georgia Institute of Technology start-up funds.

==> abstract.tex <==
\begin{abstract}

With upcoming sample return missions across the solar system and the increasing availability of mass spectrometry data, there is an urgent need for methods that analyze such data within the context of existing astrobiology literature and generate plausible hypotheses regarding the emergence of life on Earth. Hypothesis generation from mass spectrometry data is challenging due to factors such as environmental contaminants, the complexity of spectral peaks, and difficulties in cross-matching these peaks with prior studies. To address these challenges, we introduce \emph{AstroAgents}, a large language model-based, multi-agent AI system for hypothesis generation from mass spectrometry data. \emph{AstroAgents} is structured around eight collaborative agents: a data analyst, a planner, three domain scientists, an accumulator, a literature reviewer, and a critic. The system processes mass spectrometry data alongside user-provided research papers. The data analyst interprets the data, and the planner delegates specific segments to the scientist agents for in-depth exploration. The accumulator then collects and deduplicates the generated hypotheses, and the literature reviewer identifies relevant literature using Semantic Scholar. The critic evaluates the hypotheses, offering rigorous suggestions for improvement. To assess \emph{AstroAgents}, an astrobiology expert evaluated the novelty and plausibility of more than a hundred hypotheses generated from data obtained from eight meteorites and ten soil samples. Of these hypotheses, $36\%$ were identified as plausible, and among those, $66\%$ were novel\footnote{Project website: \url{https://astroagents.github.io/}}\footnote{Code is available at: \url{https://github.com/amirgroup-codes/AstroAgents}}.

\end{abstract}

==> introduction.tex <==
\section{Introduction}

The rapid growth of spectrometry data from sample return missions to the solar system, where traces of past, extinct, or present life can be found, necessitates methods to analyze this massive, high-dimensional data and generate plausible hypotheses on one of the most fundamental questions in astrobiology: How did life emerge on Earth? ~\cite{LAHAV200175, Pross2013} Analyzing mass spectrometry data in astrobiology is challenged by the presence of terrestrial contaminants \cite{Glavin2025}, the complexity of spectral peaks, and the lack of a systematic approach for hypothesis generation by comparing and contrasting to existing mass spectrometry data ~\cite{Kitano2021}. Hypothesis generation by human experts is often biased, time-consuming, and limited to the literature that the individual has expertise in~\cite{Nissen2016}. Computational methods, on the other hand, are challenged by the sparsity of peaks relevant to the dimension of the mass spectrometry data, which makes identifying patterns extremely difficult ~\cite{Guo2022}.

Recent advances in large language models (LLMs) have demonstrated remarkable capabilities in scientific reasoning ~\cite{Truhn2023} and hypothesis generation~\cite{zhou-etal-2024-hypothesis, zhang-etal-2024-comprehensive-survey}. However, these models face inherent limitations when deployed individually: They struggle with consistent reasoning over complex datasets, lack specialized domain expertise, and cannot independently validate their outputs against scientific literature ~\cite{kaddour2023challengesapplicationslargelanguage}. These limitations become particularly apparent in origins of life research, where hypotheses must bridge multiple disciplines and incorporate complex molecular evidence from mass spectrometry data.

Multi-agent architectures have emerged as a promising approach to overcoming the limitations of LLMs. Recent work has shown how multiple AI agents, each with specialized roles, can collaborate to enhance scientific discovery. \textit{SciAgents} \cite{ghafarollahi2024sciagentsautomatingscientificdiscovery} is a multi-agent AI system that combines LLMs, ontological knowledge graphs, and in-situ learning capabilities to automate scientific discovery. Similarly, \textit{HypoRefine} \cite{liu2025literaturemeetsdatasynergistic} offers an iterative approach to hypothesis refinement by synthesizing insights from scientific literature and empirical data. However, existing multi-agent systems often lack the specialized knowledge and structured workflows needed for analyzing complex mass spectrometry data in astrobiology.

\begin{figure} 
    \centering
    \includegraphics[width=1\linewidth]{images/Fig1.pdf}
    \caption{ \emph{AstroAgents} is a multi-agent system designed to generate and evaluate hypotheses about the molecular distribution of meteoritic and terrestrial samples based on mass spectrometry data. \textbf{a,} The input interface allows users to upload mass spectrometry data (in this case, coupled with gas chromatography (GC)), relevant research papers, and specific instructions to follow. \textbf{b,} The data processing agent analyzes mass spectrometry data, identifies significant patterns, detects unexpected findings, and recognizes potential environmental contamination. \textbf{c,} The planner agent delegates specific segments of the input data to a team of three scientist agents for in-depth analysis. \textbf{d,} The scientist agents generate hypotheses based on distinct aspects of the data, as assigned by the planner agent. In this illustration, the first scientist focuses on unsubstituted polycyclic aromatic hydrocarbons (PAHs), the second examines sulfur and oxygen-containing compounds, and the third investigates alkylated PAHs. \textbf{e,} The accumulator agent consolidates hypotheses generated by the scientist agents, eliminating duplicates. \textbf{f,} The literature review agent searches Semantic Scholar for relevant papers corresponding to each hypothesis and provides summarized findings. \textbf{g,} The critic agent evaluates the generated hypotheses alongside their corresponding literature reviews, offering rigorous critique and suggestions for improvement. The critic agent’s feedback is then sent to the data analyst, facilitating an iterative refinement process to enhance subsequent analyses and hypothesis generation.}
    \label{fig:fig1}
\end{figure}

Herein, we develop \emph{AstroAgents} (Fig. \ref{fig:fig1}), a multi-agent system developed to assist astrobiologists in generating hypotheses and uncovering subtle patterns within large-scale mass spectrometry datasets. \emph{AstroAgents} comprises eight specialized agents working collaboratively: a data analyst, responsible for processing mass spectrometry data, identifying significant patterns, detecting unexpected findings, and recognizing potential environmental contamination; a planner, who delegates specific segments of the input data to a team of three Scientist Agents for in-depth exploration; an accumulator agent, which consolidates hypotheses generated by the scientist agents and eliminates duplicates; a literature review agent searches Semantic Scholar \cite{Kinney2023TheSS} for relevant papers corresponding to each hypothesis and provides summarized findings; and a critic agent, which evaluates the generated hypotheses alongside their corresponding literature reviews, offering rigorous critique and suggestions for improvement. The critic agent’s feedback is then sent to the data analyst, enabling an iterative refinement process to enhance the next analyses and hypothesis generation.

We conducted two experiments using \emph{AstroAgents} powered by different large language models that varied in agentic collaboration ability \cite{vallinder2024culturalevolutioncooperationllm} and context length. In the first experiment, we used Claude Sonnet 3.5, which was supplied with 10 carefully selected research papers for astrobiological context. This configuration generated 48 hypotheses and achieved an average expert evaluation score of $6.58 \pm 1.7$ (out of $10$) while exhibiting fewer logical errors and demonstrating stronger consistency with the literature. In the second experiment, we employed Gemini 2.0 Flash, which was provided with an expanded astrobiological context comprising the same 10 research papers plus an entire book. This model produced 101 hypotheses, achieved an average score of $5.67 \pm 0.64$, and displayed a higher rate of logical errors, although it tended to generate more novel ideas. Notably, 36 of Gemini 2.0 Flash's hypotheses met the plausibility criteria, with 24 considered novel, whereas none of the hypotheses generated by Claude Sonnet 3.5 were flagged as novel. Overall, \emph{AstroAgents} is a promising step in facilitating the interpretation of mass spectrometry data and hypotheses generation.



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> method_arxiv.tex <==
\section{Methods}
In this section, we begin by outlining the user input format, then detail the responsibilities of each agent within \emph{AstroAgents}, and finally describe our approach to evaluating the quality of the generated hypotheses. For every agent, we present both the system prompt and its initial output from the first iteration. Note that these outputs were generated using Claude 3.5 Sonnet. For the complete system prompts, see the Appendix.

\subsection{User Input}

\emph{AstroAgents} begins by prompting the user to select research papers and books that are closely related to the hypotheses the domain expert aims to generate (Fig.~\ref{fig:fig1}{\bf a}). In the absence of these targeted references, the system tends to generate hypotheses that, while data-supported, are overly general. For example: 

\begin{tcolorbox}[colback=white, colframe=black]
``The presence of diverse organic compounds in meteorite samples indicates that these materials could have played a significant role in prebiotic chemistry on early Earth.''
\end{tcolorbox}

Although such a hypothesis is supported by literature, its lack of specificity diminishes its novelty. To mitigate this issue, we require users to provide relevant research papers (see Table \ref{tab:paper-context}). Each paper is then converted into the Markdown format using the \textit{pymupdf4llm} Python package, and the resulting text is used as background knowledge for the data analyst and scientist agents. Following this, users input their mass spectrometry data, which details the identified compounds and the corresponding samples in which they are found, in a LaTeX-formatted table. Finally, users provide additional instructions and detailed descriptions of the data to guide the subsequent analysis.

\subsection{Data Analyst Agent}
The data analyst agent examines mass spectrometry data to uncover key patterns, highlight anomalies, and identify potential environmental contamination (Fig. \ref{fig:fig1}\textbf{b}). It employs a structured prompt template that provides access to mass spectrometry data, astrobiological context extracted from academic papers, and user instructions. After the initial analysis, the agent refines its findings based on feedback from the critic agent.

Following the hypotheses generation phase, an accumulator agent processes the combined output from all three scientist agents (Fig. \ref{fig:fig1}\textbf{e}). This agent performs hypothesis deduplication by identifying and consolidating substantially similar hypotheses, ensuring a streamlined and non-redundant set of hypotheses for further investigation.

\clearpage

{%
    \scriptsize
    \begin{multicols}{2}
      % Left box
      \begin{tcolorbox}[
        title=Data Analyst Prompt,
        equal height group=boxes
      ]
        You are a sophisticated analytical scientist specializing in astrobiological data analysis...
        Background Context:
        
        \textbf{[SELECTED PAPERS GOES HERE]}
        Your tasks include:
        \begin{enumerate}
        \item Identifying significant patterns and trends in the dataset...
        \end{enumerate}
        Input Data:
        
        \textbf{[INPUT DATA GOES HERE]}
        
        Critic Feedback:
        
        \textbf{[CRITIC FEEDBACK GOES HERE]}
        
        Provide a refined analysis based on the above, with special emphasis on addressing critic feedback...
      \end{tcolorbox}
      
      % Right box
      \begin{tcolorbox}[
        title=Data Analyst Output,
        equal height group=boxes
      ]
        Based on the data and sample descriptions provided, I'll analyze key patterns and develop specific hypotheses,...

Key Observations and Patterns:

1. PAH Distribution Patterns: Unsubstituted PAHs (naphthalene, fluoranthene, pyrene) are predominantly found in meteorite samples...

2. Contamination Indicators: Phthalates (IDs 9, 24) appear exclusively in soil samples and newer meteorite finds ...

3. Unique Molecular Patterns: Sulfur-containing compounds (dibenzothiophene, trithiolane) appear predominantly in meteorite samples. Terpene-like compounds (IDs 4, 17, 18) are exclusively found in soil samples. Complex alkylated aromatics..

      \end{tcolorbox}
    \end{multicols}
  }

\subsection{Planner Agent}

The planner agent, based on data analysis from the data analyst agent, delegates specific segments of the input data to a team of three scientist agents for in-depth exploration (Fig. \ref{fig:fig1}{\bf c}). This agent is responsible for generating instructions for each of the three scientist agents in JSON format.

{%
    \scriptsize
    \begin{multicols}{2}
      % Left box
      \begin{tcolorbox}[
        title=Planner Prompt,
        equal height group=planner_boxes
      ]
        You are an experienced scientific planner and coordinator. Based on the data analysis provided below, your task is to delegate specific areas within the input data across a team of three scientists for in-depth exploration and investigation.

        Input Data:

        \textbf{$[$INPUT DATA GOES HERE$]$}
        
        Data Analysis:
        
        \textbf{$[$DATA ANALYST OUTPUT$]$}
        
        Your response must be ONLY a valid JSON object with the following format...
        
\begin{minted}{json}
{
    "Agent1_instructions": 
    "Detailed instructions for
    what Scientist 1 should
    focus on."
}
\end{minted}
      \end{tcolorbox}
      
      % Right box
      \begin{tcolorbox}[
        title=Planner Output,
        equal height group=planner_boxes
      ]
        \begin{minted}[breaklines]{json}
{
    "Agent1_instructions": "Focus on analyzing PAH distribution patterns in meteorite samples, specifically examining: 1) Basic PAHs like naphthalene (ID 1), fluoranthene (ID 12), and pyrene (ID 13), 2) Methylated PAHs including 2-methyl naphthalene (ID 2), 1-methyl naphthalene (ID 8), and trimethyl naphthalene (ID 15), 3) The relationship between these compounds specifically in CM2 chondrites (Murchison, ALH 83100, LON 94101)...",
}
\end{minted}
      \end{tcolorbox}
    \end{multicols}
}

\subsection{Hypothesis Generation Agents}
The expanding volume of data increasingly complicates the identification of significant patterns and relationships by individual scientists. To overcome this limitation, we developed a system that enables multiple artificial researchers to concurrently analyze different segments of data. The workflow initiates with a planner agent, which generates detailed instructions for multiple scientist agents. Each scientist agent is assigned a distinct research area and focuses on specific compound IDs for hypothesis generation. Although the number of scientist agents can exceed three, our primary objective was to demonstrate the advantage over using a single scientist agent. A single-agent approach typically concentrates exclusively on one specific research area, such as PAH molecules, thereby neglecting other molecular groups in the dataset.

Each scientist agent, operating within its assigned domain, generates hypotheses in a structured JSON format (Fig. \ref{fig:fig1}{\bf d}). Each hypothesis entry contains two key components: a statement describing the proposed hypothesis and supporting evidence in the form of key data points that substantiate the hypothesis.

\subsection{Literature Review and Critic Agent}

\emph{AstroAgents} features an integrated literature review and critique process (Fig. \ref{fig:fig1}{\bf f},{\bf g}). It utilizes the Semantic Scholar \cite{Kinney2023TheSS} to locate relevant research papers for each hypothesis, retrieving and analyzing up to five pertinent paper snippets per query. The literature review agent then processes the search results by extracting key insights, synthesizing information, and presenting a clear, concise summary while highlighting significant findings and potential conflicts.

 The critic agent evaluates each hypothesis based on its consistency with experimental data, scientific rigor, theoretical basis from the selected papers, and integration with external literature gathered by literature review agents. The critic particularly focuses on assessing the novelty and specificity of the claims, providing structured feedback to guide the next round of hypothesis refinement. Finally, the critic's response is passed to the Data Analyst agent for further iterative improvements.



{%
    \scriptsize
    \begin{multicols}{2}
      % Left box
      \begin{tcolorbox}[
        title=Scientist Prompt,
        equal height group=scientist_boxes
      ]
        You are a sophisticated astrobiologist and prebiotic chemist specializing in meteoritic organic compounds.

You are Scientist \textbf{AGENT\_ID}. 

Instructions: \textbf{AGENT\_INSTRUCTION}.

IMPORTANT: Only focus on the data that is assigned to you.

Background Context: \textbf{$[$SELECTED PAPERS$]$}

Input Data: \textbf{$[$INPUT DATA $]$}

Based on the above, generate new hypotheses and conclusions as necessary.
You must respond ONLY with a valid JSON object in the following format, with no additional text before or after:
\begin{minted}[breaklines]{json}
{
    "id": "Format it like H_one, H_two, etc.",
    "statement": "Explain the hypothesis fully and in detail here.",
    "key_datapoints": "List of compounds and samples that support the hypothesis, directly point to ID or compound/sample name.",
}

\end{minted}
      \end{tcolorbox}
      
      % Right box
      \begin{tcolorbox}[
        title=Scientist 1 Output,
        equal height group=scientist_boxes
      ]
        \begin{minted}[breaklines]{json}
[{
"id": "H_one",
"statement": "The presence of methylated naphthalenes (2-methyl naphthalene, 1-methyl naphthalene, trimethyl naphthalene) exclusively in meteorite samples but not in soil samples suggests that alkylation of PAHs occurs through abiotic processes in space rather than through biological activity.",
"key_datapoints": "IDs 2, 8, 15 found in meteorites (Orgueil, ALH 83100, LON 94101, Murchison, Jbilet Winselwan, LEW 85311) but absent in all soil samples"
},
{
"id": "H_two", 
"statement": "The co-occurrence of fluoranthene and pyrene (IDs 12,13) specifically in Antarctic meteorites suggests these..."
}]
\end{minted}
      \end{tcolorbox}
    \end{multicols}
}

{%
    \scriptsize
    \begin{multicols}{2}
      % Left box
      \begin{tcolorbox}[
        title=Literature Review Prompt,
        equal height group=literature_review_boxes
      ]
        You are a specialized literature review agent analyzing scientific literature search results.

Your tasks include:
\begin{enumerate}
    \item Analyzing the search results provided below.
    \item Extracting and synthesizing key insights.
    \item Formatting your summary clearly and concisely.
    \item Highlighting significant findings and noting any conflicting evidence.
\end{enumerate}

Query:

\textbf{[THE LIST OF HYPOTHESES GOES HERE]}

Search Results:

\textbf{[SEARCH RESULTS GOES HERE]}
      \end{tcolorbox}
      
      % Right box
      \begin{tcolorbox}[
        title=Literature Review Output,
        equal height group=literature_review_boxes
      ]

\textbf{Hypothesis H\_final\_one:}
Here's my analysis of the search results regarding methylated naphthalenes in meteorites versus soil samples:

Key Findings: 1. Origin and Formation:PAHs are generally not produced by living organisms and are "essentially in...

===

\textbf{Hypothesis H\_final\_two:}
Here's my synthesized analysis of the search results regarding the co-occurrence of fluoranthene and pyrene in Antarctic meteorites:

\textbf{Key Findings:}
1. Formation Mechanisms \& Conditions
- Recent isotopic analysis of asteroid Ryugu suggests that two- and four-ring PAHs (including fluoranthene and pyrene) likely formed in low-temperature interstellar environments...
      \end{tcolorbox}
    \end{multicols}
}


{
    \scriptsize
    \begin{multicols}{2}
      % Left box
      \begin{tcolorbox}[
        title=Critic Prompt,
        equal height group=critic_boxes
      ]
You are an expert scientist in astrobiology and prebiotic chemistry, with deep expertise in PAH analysis and meteoritic organic chemistry.

Background Context:

\vspace{3mm}

\textbf{[SELECTED PAPERS]}

\vspace{3mm}

Your task is to provide a detailed, scientifically rigorous critique of the proposed hypothesis and the associated data analysis...

Your critique must include:

\begin{enumerate}
    \item Alignment with the data...
\end{enumerate}

Input Data:

\vspace{3mm}

\textbf{[INPUT DATA]}

\vspace{3mm}

Literature Review:

\vspace{3mm}

\textbf{[LITERATURE REVIEW GOES HERE]}

\vspace{3mm}

Hypothesis:

\vspace{3mm}

\textbf{[ACCUMULATED HYPOTHESES GOES HERE]}

\vspace{3mm}
      \end{tcolorbox}
      
      % Right box
      \begin{tcolorbox}[
        title=Critic Output,
        equal height group=critic_boxes
      ]
Thank you for providing the detailed hypotheses and data. I'll provide a structured critique of each hypothesis:

\vspace{1mm}
\textbf{H\_final\_one - Methylated Naphthalenes:}

\textbf{Strengths:}

- Clear correlation between methylated naphthalenes and meteoritic samples...

\textbf{Critical Weaknesses:}
\begin{enumerate}
    \item Oversimplified causation - The exclusive presence in meteorites doesn't necessarily prove abiotic formation
    \item Ignores potential preservation bias - Methylated naphthalenes may form biologically but preserve better in meteoritic matrices ...
\end{enumerate}

\textbf{H\_final\_two - Fluoranthene/Pyrene:}

\textbf{Critical Flaws:}

1. Correlation $\neq$ Causation - Co-occurrence doesn't prove similar formation mechanisms

2. Sample bias - Only examines Antarctic meteorites

3. Ignores temperature history - Antarctic storage conditions may affect PAH distributions

4. No mechanistic evidence provided for ion-molecule reactions

\textbf{This hypothesis should be rejected due to insufficient evidence.}

      \end{tcolorbox}
    \end{multicols}
}

